Generation, propagation and control of quantized vortices and dark solitons in polariton superfluids

Exciton-polaritons are quasi-particles arising from the strong coupling regime between excitons and photons. In planar microcavitites, phenomena such as superfluidity or Bose-Einstein condensation can be observed. Those systems have demonstrated to be very efficient in the hydrodynamic generation of topological excitations, such as vortex-antivortex pairs or dark solitons. However, the lifetime and motion of those excitations were limited by the driven dissipative nature of the system. In this thesis, we present a rich variety of results about the generation and control of such topological excitations. Taking advantage of the optical bistability present in our system, we were able to greatly enhanced the propagation length of vortices and solitons generated in the wake of a structural defect, revealing in the mean time an unexpected binding mechanism of the solitons which propagate parallel. This behaviour was recovered in a specifically designed experiment, where we artificially imprint dark soliton pairs on demand on a polariton superfluid. The adaptability of our technique allowed for a detailed study of this phenomenon, that we directly connected to the driven-dissipative nature of our system. Finally, confined dark solitons were generated within guided intensity channels on a static polariton fluid. The absence of flow lead to the development of transverse snake instabilities of which we studied the interesting properties.

==> thcoverdata.tex <==
%!TeX encoding = UTF-8
% Metadata for coverpages
\thesisname{Thèse de doctorat}
\gradename{docteur}
\univ{de Sorbonne Université}
\logos{SorbonneUniv.png}{LKB.pdf}{CNRS.pdf}                   % Un à trois logo. Le 1er est celui de \univ
\specialite{Physique}
\ecoledoctnum{564}
\ecoledoct{Physique en Île-de-France}
\title{Generation, propagation and control of quantized vortices and dark solitons in polariton superfluids}
\titleen{Génération, propagation et contrôle de vortex quantifiés et solitons sombres dans des superfluides de polaritons}

% si nécessaire, pour les métadonnées
%\titlemeta{La laine des Dupondt au Pays de l'or noir} 
%\titlemetaen{Dupondt's wool in "Land of Black Gold" } 

\date{27/11/2020}
\author{Anne MA\^{I}TRE}
\advisor{Alberto BRAMATI}
\atinstitution{à Sorbonne Université}
\atlab{{\Large au Laboratoire Kastler Brossel}}
% Jury as LaTeX Tabular. Pas de président avant soutenance								  
\jury{ %                         
Mme & Maria CHAMARRO & Examinatrice           \\
M. & Cristiano CIUTI & Examinateur           \\
M. & Massimo GIUDICI & Rapporteur        \\
M. & Thierry GUILLET & Rapporteur        \\
M. & Pavlos SAVVIDIS & Examinateur         \\
M. & Alberto BRAMATI & Directeur de thèse      \\
M. & Simon PIGEON & Invité}
\makeatletter
\@ifpackageloaded{thcover-psl}{\logos{PSL}{LKB}{}}{\relax}
\makeatother

\resume{Exciton-polaritons are quasi-particles arising from the strong coupling regime between excitons and photons. In planar microcavitites, phenomena such as superfluidity or Bose-Einstein condensation can be observed. Those systems have demonstrated to be very efficient in the hydrodynamic generation of topological excitations, such as vortex-antivortex pairs or dark solitons. However, the lifetime and motion of those excitations were limited by the driven dissipative nature of the system.

\paragraph{}
In this thesis, we present a rich variety of results about the generation and control of
such topological excitations. Taking advantage of the optical bistability present in our system, we were able to greatly enhanced the propagation length of vortices and solitons generated in the wake of a structural defect, revealing in the mean time an unexpected binding mechanism of the solitons which propagate parallel.
This behaviour was recovered in  a specifically designed  experiment, where we artificially imprint dark soliton pairs on demand on a polariton superfluid. The adaptability of our technique allowed for a detailed study of this phenomenon, that we directly connected to the driven-dissipative nature of our system.
Finally, confined dark solitons were generated within guided intensity channels on a static polariton fluid. The absence of flow lead to the development of transverse snake instabilities of which we studied the interesting properties.
}

\motscles{fluid of light, exciton-polaritons, quantum vortices, dark solitons, snake instabilities.}

% si nécessaire, pour les métadonnées
%\titlemetaen{Dupondt's wool in "Land of Black Gold" } 

\abstract{Les polaritons excitoniques sont des quasi-particules créées par le régime de couplage fort entre des excitons et des photons. Dans des microcavités planaires, des phénomènes tels que la superfluidité ou la condensation de Bose-Einstein ont pu être observés.
Ces systèmes ont démontrés être particulièrement appropriés pour la génération hydrodynamique d'excitations topologiques comme des paires de vortex-antivortex ou de solitons sombres.
Cependant, le temps de vie et la propagation de ces excitations étaient limités par la dissipation du système.

\paragraph{}
Dans cette thèse, nous présentons une succession de résultats sur la génération et le contrôle de telles excitations topologiques. 
En utilisant la bistabilité optique de notre système, nous avons fortement augmenté la distance de propagation de vortex et de solitons formés dans le sillage de défauts structurels, ce qui a également révélé un comportement inattendu des solitons liés qui restent parallèles.
Ce comportement a été confirmé par l’expérience suivante, où nous avons artificiellement imprimé des paires de solitons sombres dans des superfluides de polaritons. 
La flexibilité de notre technique nous a permis d'étudier ce phénomène en détails et de le relier directement à la dissipation du système.
Enfin, des solitons sombres ont été produits dans des canaux d'intensités dans un fluide statique. L'absence de flux a permis le développement d'instabilités transverses ou \textit{snake instabilities} dont nous avons étudié les propriétés.
% Alors que les photons dans le vide sont des particules qui n'intéragissent pas entre elles,
}

\keywords{fluide de lumière, polaritons excitoniques, vortex quantifiés, solitons sombres, instabilités}


